Pose-MUM : Reinforcing Key Points Relationship for Semi-Supervised Human Pose Estimation

A well-designed strong-weak augmentation strategy and the stable teacher to generate reliable pseudo labels are essential in the teacher-student framework of semi-supervised learning (SSL). Considering these in mind, to suit the semi-supervised human pose estimation (SSHPE) task, we propose a novel approach referred to as Pose-MUM that modifies Mix/UnMix (MUM) augmentation. Like MUM in the dense prediction task, the proposed Pose-MUM makes strong-weak augmentation for pose estimation and leads the network to learn the relationship between each human key point much better than the conventional methods by adding the mixing process in intermediate layers in a stochastic manner. In addition, we employ the exponential-moving-average-normalization (EMAN) teacher, which is stable and well-suited to the SSL framework and furthermore boosts the performance. Extensive experiments on MS-COCO dataset show the superiority of our proposed method by consistently improving the performance over the previous methods following SSHPE benchmark.

==> tables/ablation_study.tex <==
\begin{table*}
\caption{
Ablation results of HDML on CUB-200-2011 and CARS-196 datasets.
% Ablation results: Impact of each component. For all results, embedding size is fixed by 512.
}
\label{ablation}
\centering
\scriptsize
% \tiny
\begin{tabular}{
p{0.11\textwidth}
>{\centering}p{0.09\textwidth}
>{\centering}p{0.09\textwidth}
>{\centering}p{0.09\textwidth}
>{\centering}p{0.09\textwidth}
>{\centering}p{0.12\textwidth}
>{\centering\arraybackslash}p{0.12\textwidth}
}
\toprule
    \multirow{2}{*}{Model}
    & \multicolumn{2}{c}{Representative}
    & \multicolumn{2}{c}{Classification}
    & \multirow{2}{*}{CUB-200-2011}
    & \multirow{2}{*}{CARS-196}
    \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
    & Centroid
    & Distribution
    & Sample
    & Hypergraph
    &  (R@1)
    &  (R@1)
    \\

\midrule

    %%% variant 1.
    M1 (Baseline)
        & \cmark
        & -
        & \cmark
        & -
        & 67.4 $\pm$ 0.3
        & 86.6 $\pm$ 0.5
        \\
    
    %%% variant 2.
    M2
        & -
        & \cmark
        & \cmark
        & -
        & 68.2 $\pm$ 0.2
        & 87.0 $\pm$ 0.2
        \\
        

    %%% variant 3.
    M3
        & \cmark
        & -
        & -
        & \cmark
        & 68.4 $\pm$ 0.4
        & 87.3 $\pm$ 0.3
        \\

    %%% variant 4.
    M4 (Proposed)
        & -
        & \cmark
        & -
        & \cmark
        & \textbf{71.4 $\pm$ 0.2}
        & \textbf{89.6 $\pm$ 0.2}
        \\
    

\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table*}

==> tables/alpha.tex <==
\begin{table}
\caption{Recall@1 (\%) comparison among different $\alpha$ values on CAR-196 dataset.
}
\label{alpha}
\centering
\scriptsize
% \tiny
\begin{tabular}{
ccc
}
\toprule
    $\alpha$
    & Hyperedge
    & R@1
    \\
\midrule

    0.0
        & All sample
        & 87.7 $\pm$ 0.2
        \\
    
    0.6
        & \tikzmark{a}
        & 88.4 $\pm$ 0.3
        \\
    
    0.9
        & 
        & \textbf{89.6 $\pm$ 0.2}
        \\
    
    1.2
        & 
        & 88.8 $\pm$ 0.2
        \\
    
    2.0
        & \tikzmark{b}
        & 87.7 $\pm$ 0.3
        \\
    
    $\infty$ 
        & Binary
        & 88.1 $\pm$ 0.3
        \\
    
\bottomrule
\end{tabular}
\tikz[remember picture, overlay] \draw[->] (a.center -| b.center) -- (b.center);
\end{table}

==> tables/choice_batch_sampler.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{ccc}
    \toprule
    Batch sampling
    & CUB-200-2011
    & CARS-196
    \\
    
    \midrule
    \midrule

    Random (32)
        & 71.4 $\pm$ 0.2
        & \textbf{89.6 $\pm$ 0.2}
        \\
        
    Balanced ($4 \times 8$)
        & \textbf{71.7 $\pm$ 0.2}
        & 89.1 $\pm$ 0.3
        \\
    
    \bottomrule
\end{tabular}
\caption{Robustness to \textit{unseen} input deformations. We evaluated Recall@1 (\%) performance with different input deformations on CAR-196 dataset.
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{choice-batch-sampler}
\end{table}

==> tables/choice_batch_size.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{ccc}
    \toprule
    Batch size
    & Memory
    & R@1
    \\
    
    \midrule
    \midrule

    32
        &
        & 89.6 $\pm$ 0.2
        \\
        
    48
        &
        & 88.9 $\pm$ 0.3
        \\
        
    64
        &
        & \textbf{89.7 $\pm$ 0.3}
        \\
        
    80
        &
        & 88.1 $\pm$ 0.2
        \\
        
    96
        &
        & 87.8 $\pm$ 0.3
        \\

    \bottomrule
\end{tabular}
\caption{Robustness to \textit{unseen} input deformations. We evaluated Recall@1 (\%) performance with different input deformations on CAR-196 dataset.
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{choice-batch-size}
\end{table}

==> tables/datasets.tex <==
\begin{table}
\caption{Dataset statistics.}
\label{datasets}
\centering
\scriptsize
\begin{tabular}{
p{0.13\textwidth}
>{\centering}p{0.08\textwidth}
>{\centering}p{0.08\textwidth}
>{\centering}p{0.08\textwidth}
>{\centering\arraybackslash}p{0.08\textwidth}
}
\toprule
    \multirow{2}{*}{Name}
    & \multicolumn{2}{c}{Num. of Images}
    & \multicolumn{2}{c}{Num. of Classes}
    \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
    & Train
    & Test
    & Train
    & Test
    \\

\midrule

CUB-200-2011
    & 5,864
    & 5,924
    & 100
    & 100
    \\

CARS-196
    & 8,054
    & 8,131
    & 98
    & 98
    \\
    
SOP
    & 59,551
    & 60,502
    & 11,318
    & 11,316
    \\

\bottomrule
\end{tabular}
\end{table}

==> tables/effect_HIST.tex <==
\begin{table}
\centering
\footnotesize
{
\begin{tabular}{llc} 
    \toprule
    Method
    & Relations
    & R@1
    \\
    
    \midrule
    \midrule
    
    \multicolumn{3}{l}{\textit{\textbf{Single classification:}}}
    \\
    
    Baseline
        & -
        & 86.4 $\pm$ 0.2
        \\
    
    \midrule
    
    \multicolumn{3}{l}{\textit{\textbf{Graph-based classification:}}}
    \\
    
    % G-Sim
    %     & Feature similarity
    %     & 00.0 $\pm$ 0.0
    %     \\
        
    TF-like
        & Transformer~\cite{vaswani2017attention}-like attention
        & 87.6 $\pm$ 0.3
        \\
    
    % GL~\cite{elezi2020group}$^{\dagger}$  % ECCV'20
    %     & I
    %     & Similarity graph + LP
    %     & 85.6
    %     \\
    
    % P.GML~\cite{Zhu2020ProxyGML}$^{\dagger}$ % NeurIPS'20
    %     & I
    %     & Bipartite graph (data-proxy)
    %     & 85.5
    %     \\
    
    % IBC~\cite{seidenschwarz2021learning}$^{\dagger}$  % ICML'21
    %     & R50
    %     & Transformer~\cite{vaswani2017attention}-like MPNs
    %     & 88.1
    %     \\
    
    \midrule
    
    \multicolumn{3}{l}{\textit{\textbf{Hypergraph-based classification:}}}
    \\
    H-Pos
        & Only positive samples
        & 87.4 $\pm$ 0.2
        \\ 
    
    % H-All
    %     & All samples
    %     & 00.0 $\pm$ 0.0
    %     \\
    
    HIST (w.o. $\mathcal{L}_D$)
        & Semantic tuplets
        & 88.3 $\pm$ 0.2
        \\
    
    \rowcolor{Gray}
    HIST
        & Semantic tuplets
        & \textbf{89.6 $\pm$ 0.2}
        \\
    
    % \midrule 
    
    % HIST \scalebox{0.9}{($\alpha=0.6$)}
    %     & R50
    %     & Semantic tuplets
    %     & 88.3 $\pm$ 0.3
    %     \\
    
    % \rowcolor{Gray}
    % HIST \scalebox{0.9}{($\alpha=0.9$)}
    %     & R50
    %     & Semantic tuplets
    %     & \textbf{89.6 $\pm$ 0.2}
    %     \\
    
    % HIST \scalebox{0.9}{($\alpha=1.2$)}
    %     & R50
    %     & Semantic tuplets
    %     & 88.8 $\pm$ 0.2
    %     \\
    
    % HIST \scalebox{0.9}{($\alpha=2.0$)}
    %     & R50
    %     & Semantic tuplets
    %     & 88.1 $\pm$ 0.3
    %     \\
    
    \bottomrule

\end{tabular}
}
\vspace{-1mm}
\caption{Retrieval performance of ablation models on CARS-196.
% Superscript denotes the embedding dimension.
% %
% For all compared methods, the results are quoted from the original paper.
% %
% The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{effect-hist}
\end{table}




==> tables/effect_component.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{lcc}
    \toprule
    Method
    & CUB-200-2011
    & CARS-196
    \\
    
    \midrule
    \midrule
    
    HIST (w.o. $\mathcal{L}_D$)
        & 00.0 $\pm$ 0.0
        & 00.0 $\pm$ 0.0
        \\
    
    HIST (w.o. covariance)
        & 68.4 $\pm$ 0.4
        & 87.3 $\pm$ 0.3
        \\
    
    HIST
        & \textbf{71.4 $\pm$ 0.2}
        & \textbf{89.6 $\pm$ 0.2}
        \\
    
    \bottomrule
\end{tabular}
\caption{Robustness to \textit{unseen} input deformations. We evaluated Recall@1 (\%) performance with different input deformations on CAR-196 dataset.
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{effect-component}
\end{table}

==> tables/res_64dim.tex <==
\begin{table}
\caption{Image retrieval and clustering performances (\%) on CUB-200-2011, CARS-196, and SOP datasets. 
%  
우리는 10번 반복실험. 괄호 안의 숫자는 95\% confidence interval 의 margin of error. 
%
For all compared methods, the results are quoted from the original paper.
% , and "-" means that the result is not provided.
Superscript denotes the embedding size.
% , and "$\dagger$" indicates that the model uses a larger input image.
% The top-3 results are shown in bold, with the best in red, the second-best in blue, and the third-best in black.
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{result-64dim}
\centering
% \scriptsize
\tiny
{
\begin{tabular}{
p{0.155\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering\arraybackslash}p{0.0375\textwidth}
} 
    \toprule
    \multirow{2}{*}{Method}
    &  \multicolumn{4}{c}{CUB-200-2011}
    &  \multicolumn{4}{c}{CARS-196}
    &  \multicolumn{4}{c}{SOP}
    \\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    \cmidrule(l){10-13}
    & R@1 & R@2 & R@4 & R@8 
    & R@1 & R@2 & R@4 & R@8 
    & R@1 & R@10 & R@10$^{\text{2}}$ & R@10$^{\text{3}}$
    \\
    \midrule

    % \textbf{64-\textit{dimension}} 
    % & & & & 
    % & & & & 
    % & & & & 
    % \\
    
    LiftStruct$^{\text{64}}$~\cite{oh2016deep} % CVPR'16
        % CUB-200-2011
        & 43.6 
        & 56.6 
        & 68.6
        & 
        % CARS-196
        & 53.0 
        & 65.7 
        & 76.0
        & 
        % SOP
        & 62.5 
        & 80.8 
        & 91.9
        & 
        \\
    
    N-pair-mc$^{\text{64}}$~\cite{sohn2016improved} % NeurIPS'16... multi-scale test (softtriple 논문 참고)
        % CUB-200-2011
        & 51.0
        & 63.3
        & 74.3
        & 
        % CARS-196
        & 71.1
        & 79.7
        & 86.5
        & 
        % SOP
        & 67.7
        & 83.8
        & 93.0
        & 
        \\
    
    Clustering$^{\text{64}}$~\cite{oh2017deep} % CVPR'17
        % CUB-200-2011
        & 48.2 
        & 61.4
        & 71.8
        & 
        % CARS-196
        & 58.1 
        & 70.6 
        & 80.3
        & 
        % SOP
        & 67.0 
        & 83.7
        & 93.2
        & 
        \\
        
    ProxyNCA$^{\text{64}}$~\cite{movshovitz2017no} % ICCV'17
        % CUB-200-2011
        & 49.2
        & 61.9
        & 67.9
        & 
        % CARS-196
        & 73.2 
        & 82.4 
        & 86.4
        & 
        % SOP
        & 73.7
        & -
        & -
        & 
        \\
        
    % $^{\dagger}$Margin$^{128}$~\cite{wu2017sampling} % ICCV'17
    %     % CUB-200-2011
    %     & 63.6 
    %     & 74.4 
    %     & 83.1 
    %     & 69.0
    %     % CARS-196
    %     & 79.6 
    %     & 86.5 
    %     & 91.9
    %     & 69.1
    %     % SOP
    %     & 72.7 
    %     & 86.2 
    %     & 93.8
    %     & 90.7
    %     \\
    
    SoftTriple$^{\text{64}}$~\cite{qian2019softtriple} % ICCV'19
        % CUB-200-2011
        & 60.1
        & 71.9
        & 81.2
        & 
        % CARS-196
        & 78.6
        & 86.6
        & 91.8
        & 
        % SOP
        & 76.3
        & 89.1
        & 95.3
        & 
        \\
    
    ProxyAnchor$^{\text{64}}$~\cite{kim2020proxy} % CVPR'20
        % CUB-200-2011
        & 61.7
        & 73.0
        & 81.8
        & 
        % CARS-196
        & 78.8
        & 87.0
        & \textbf{92.2}
        & 
        % SOP
        & 76.5
        & 89.0
        & 95.1
        & 
        \\
    
    ProxyGML$^{\text{64}}$~\cite{Zhu2020ProxyGML} % NeurIPS'20
        % CUB-200-2011
        & 59.4
        & 70.1
        & 80.4
        & 
        % CARS-196
        & 78.9
        & 87.5
        & 91.9
        & 
        % SOP
        & 76.2
        & 89.4
        & 95.4
        & 
        \\
    
    \midrule
    
    HDML$^{\text{64}}$
        % CUB-200-2011
        & \textbf{63.6} \tiny{(0.0)}
        & \textbf{74.9}
        & \textbf{83.6}
        & 
        % CARS-196
        & 
        & 
        & 
        & 
        % SOP
        & 
        & 
        & 
        & 
        \\
    
    \bottomrule
\end{tabular}
}
\end{table}



==> tables/res_backbone.tex <==
\begin{table}
\caption{같은 backbone 쓰는 방법들끼리의 비교. Recall@1 comparisons. For all results, embedding size 는 512 로 fixed. 여러가지 backbone 에 대해 모두 실험을 한 방법들의 경우 그 중 가장 best 성능을 기록하였다. MS+SEC, MDR, PS 는 기존 방법들에 add-on 되어서 combination 되는 것들. 이들은 기존 방법에 추가적으로 add-on 하여 performance improvement 가 있다고 주장하는 논문들... (additional training technique with multi-distance regularization), ps (data augmentation with synthetic classes and embeddings) 이 추가됨. 이런 것 없이도 compatible 한 결과를 얻음. fair 한 비교를 위해 아예 이 표에서 뺄까?}
\label{result-backbone}
\centering
\scriptsize
\begin{tabular}{
p{0.15\textwidth}
>{\centering}p{0.12\textwidth}
>{\centering}p{0.15\textwidth}
>{\centering\arraybackslash}p{0.15\textwidth}
}
\toprule
    Method
    & Backbone 
    & CUB-200-2011
    & CARS-196
    \\
    
\midrule
    Pre-trained~\cite{musgrave2020metric}
    & \multirow{4}{*}{GoogleNet} 
    & 41.1
    & 33.9
    \\
    
    
    DVML~\cite{lin2018deep} % ECCV'18
    & 
    & 52.7
    & 82.0
    \\
    
    ABE-8~\cite{kim2018attention} % ECCV'18
    &
    & \underline{60.6}
    & \underline{85.2}
    \\
    
    HDML
    &
    & \textbf{00.0 $\pm$ 0.0}
    & \textbf{00.0 $\pm$ 0.0}
    \\
    
\midrule
    
    Pre-trained~\cite{musgrave2020metric}
    & \multirow{11}{*}{BN-Inception}
    & 51.1 
    & 46.9 
    \\
    
    HTL~\cite{ge2018deep} % ECCV'18
    & 
    & 57.1 
    & 81.4 
    \\
    
    RLL-H~\cite{wang2019ranked} % CVPR'19
    &
    & 57.4
    & 74.0
    \\
    
    MS~\cite{wang2019multi} % CVPR'19
    & 
    & 65.7 
    & 84.1
    \\
    
    
    SoftTriple~\cite{qian2019softtriple} % ICCV'19
    &  
    & 65.4
    & 84.5
    \\
    
    CircleLoss~\cite{sun2020circle}     % CVPR'20
    & 
    & 66.7
    & 83.4
    \\
    
    ProxyAnchor~\cite{kim2020proxy}     % CVPR'20
    &
    & 68.4
    & 86.1
    \\
    
    ProxyGML~\cite{Zhu2020ProxyGML}     % NeurIPS'20
    &
    & 66.6
    & 85.5
    \\
    
    MS+SEC~\cite{zhang2020deep}  % NeurIPS'20
    & 
    & 68.8
    & 85.7
    \\
    
    PS+PA~\cite{gu2021proxy}  % AAAI'21
    &
    & \underline{69.2} 
    & \underline{86.9}
    \\
    
    HDML
    &
    & \textbf{69.6 $\pm$ 0.3}
    & \textbf{87.2 $\pm$ 0.0}
    \\
    
\midrule
    
    Pre-trained~\cite{musgrave2020metric}
    & \multirow{6}{*}{ResNet50}
    & 48.7
    & 43.5
    \\
    
    N.Softmax~\cite{zhai2018classification} % BMVC'19
    & 
    & 61.3
    & 84.2
    \\
    
    ProxyNCA\tiny{++}~\cite{teh2020proxynca++}  % ECCV'20
    &  
    & 64.7
    & 85.1
    \\
    
    DiVA~\cite{milbich2020diva}    % ECCV'20
    &
    & 69.2
    & 87.6
    \\
    
    ProxyAnchor~\cite{kim2020proxy}     % CVPR'20
    &
    & \underline{69.7}
    & \underline{87.7}
    \\
    
    HDML
    &
    & \textbf{71.4 $\pm$ 0.2}
    & \textbf{89.6 $\pm$ 0.2}
    \\
    
\bottomrule
\end{tabular}
\end{table}




==> tables/res_cub_cars_sop.tex <==
\begin{table*}[t]
\centering
\scriptsize
{
\begin{tabular}{lcccccccccccc} 
    \toprule
    \multirow{2}{*}{Method}
    &  \multicolumn{4}{c}{CUB-200-2011}
    &  \multicolumn{4}{c}{CARS-196}
    &  \multicolumn{4}{c}{SOP}
    \\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    \cmidrule(l){10-13}
    & R@1 & R@2 & R@4 & NMI 
    & R@1 & R@2 & R@4 & NMI 
    & R@1 & R@10 & R@100 & NMI
    \\
    \midrule
    \midrule
    
    \multicolumn{5}{l}{\textit{\textbf{Methods using BN-Inception:}}}
    & & & &
    & & & &
    \\
    
    HTL$^{512}$~\cite{ge2018deep} % ECCV'18
        % CUB-200-2011
        & 57.1 
        & 68.8 
        & 78.7
        & -
        % CARS-196
        & 81.4 
        & 88.0
        & 92.7
        & -
        % SOP
        & 74.8
        & 88.3
        & 94.8
        & -
        \\
    
    RLL-H$^{512}$~\cite{wang2019ranked} % CVPR'19
        % CUB-200-2011
        & 57.4
        & 69.7
        & 79.2
        & 63.6
        % CARS-196
        & 74.0
        & 83.6
        & 90.1
        & 65.4
        % SOP
        & 76.1
        & 89.1
        & 95.4
        & 89.7
        \\
        
    MS$^{\text{512}}$~\cite{wang2019multi} % CVPR'19
        % CUB-200-2011
        & 65.7 
        & 77.0
        & 86.3
        & -
        % CARS-196
        & 84.1 
        & 90.4 
        & 94.0
        & -
        % SOP
        & 78.2 
        & 90.5 
        & 96.0
        & -
        \\
    
    SoftTriple$^{\text{512}}$~\cite{qian2019softtriple} % ICCV'19
        % CUB-200-2011
        & 65.4
        & 76.4
        & 84.5 
        & 69.3
        % CARS-196
        & 84.5 
        & 90.7 
        & 94.5
        & 70.1
        % SOP
        & 78.3
        & 90.3
        & 95.9
        & \underline{92.0}
        \\
    
    GroupLoss$^{\text{1024}}$~\cite{elezi2020group}      % ECCV'20
        % CUB-200-2011
        & 65.5
        & 77.0
        & 85.0
        & 69.0
        % CARS-196
        & 85.6
        & 91.2
        & 94.9
        & \underline{72.7}
        % SOP
        & 75.7
        & 88.2
        & 94.8
        & 91.1
        \\
    
    CircleLoss$^{\text{512}}$~\cite{sun2020circle} % CVPR'20
        % CUB-200-2011
        & 66.7
        & 77.4
        & 86.2
        & -
        % CARS-196
        & 83.4
        & 89.8
        & 94.1
        & -
        % SOP
        & 78.3
        & 90.5
        & \underline{96.1}
        & -
        \\
    
    ProxyAnchor$^{\text{512}}$~\cite{kim2020proxy} % CVPR'20
        % CUB-200-2011
        & 68.4
        & 79.2
        & 86.8
        & -
        % CARS-196
        & 86.1
        & 91.7
        & 95.0
        & -
        % SOP
        & \underline{79.1}
        & \underline{90.8}
        & \textbf{96.2}
        & -
        \\
    
    ProxyGML$^{\text{512}}$~\cite{Zhu2020ProxyGML} % NeurIPS'20
        % CUB-200-2011
        & 66.6 
        & 77.6
        & 86.4
        & \underline{69.8}
        % CARS-196
        & 85.5 
        & 91.8
        & \underline{95.3}
        & 72.4
        % SOP
        & 78.0
        & 90.6
        & \textbf{96.2}
        & 90.2
        \\
    
    % SEC$^{\text{512}}$~\cite{zhang2020deep}  % NeurIPS'20
    %     % CUB-200-2011
    %     & 68.8
    %     & 79.4
    %     & \underline{87.2}
    %     & 72.9
    %     % CARS-196
    %     & 85.7 
    %     & 92.0
    %     & \underline{95.5}
    %     & 74.0
    %     % SOP
    %     & 78.7 
    %     & 90.8 
    %     & \underline{96.2}
    %     & 91.9
    %     \\
    
    DRML$^{\text{512}}$~\cite{zheng2021relational}  % ICCV'21
        % CUB-200-2011
        & 68.7 
        & 78.6
        & 86.3
        & 69.3
        % CARS-196
        & \underline{86.9}
        & \underline{92.1}
        & 95.2
        & 72.1
        % SOP
        & 71.5
        & 85.2
        & 93.0
        & 88.1
        \\
        
    DAM$^{\text{512}}$~\cite{xu2021discrimination}  % CVPR'21
        % CUB-200-2011
        & \underline{69.1} 
        & \underline{79.8}
        & \underline{87.2}
        & -
        % CARS-196
        & \underline{86.9}
        & \underline{92.1}
        & \underline{95.3}
        & -
        % SOP
        & -
        & -
        & -
        & -
        \\

    \rowcolor{Gray}  
    % \midrule
    HIST$^{\text{512}}$ (Ours)
        % CUB-200-2011
        & \textbf{69.7}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.3}
        & \textbf{80.0}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{87.3}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{70.8}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        % CARS-196
        & \textbf{87.4}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{92.5}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.3}
        & \textbf{95.4}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        & \textbf{73.0}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        % SOP
        & \textbf{79.6}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{91.0}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{96.2}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{92.2}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.3}
        \\    

    \midrule
    % \midrule
    
    \multicolumn{5}{l}{\textit{\textbf{Methods using ResNet-50:}}}
    & & & &
    & & & &
    \\
    
    N.Softmax$^{512}$~\cite{zhai2018classification} % BMVC'19
        % CUB-200-2011
        & 61.3 
        & 73.9
        & 83.5
        & 69.7
        % CARS-196
        & 84.2
        & 90.4 
        & 94.4
        & 74.0
        % SOP
        & 78.2 
        & 90.6
        & \underline{96.2}
        & 91.0
        \\
    
    FastAP$^{\text{512}}$~\cite{cakir2019deep} % CVPR'19
        % CUB-200-2011
        & - 
        & -
        & -
        & -
        % CARS-196
        & - 
        & -
        & -
        & -
        % SOP
        & 76.4 
        & 89.0 
        & 95.1 
        & -
        \\
        
    TML$^{\text{512}}$~\cite{yu2019deep} % ICCV'19
        % CUB-200-2011
        & 62.5 
        & 73.9 
        & 83.0
        & -
        % CARS-196
        & 86.3 
        & 92.3 
        & 95.4
        & -
        % SOP
        & 78.0 
        & 91.2 
        & \textbf{96.7} 
        & -
        \\
    
    ProxyAnchor$^{\text{512}}$~\cite{kim2020proxy} % CVPR'20
        % CUB-200-2011
        & 69.7
        & 80.0
        & 87.0
        & -
        % CARS-196
        & 87.7
        & 92.9
        & 95.8
        & -
        % SOP
        & -
        & -
        & -
        & -
        \\
    
    ProxyNCA++$^{\text{512}}$~\cite{teh2020proxynca++} % ECCV'20
        % CUB-200-2011
        & 64.7
        & -
        & -
        & -
        % CARS-196
        & 85.1
        & -
        & -
        & -
        % SOP
        & 79.6
        & -
        & -
        & -
        \\
    
    DiVA$^{512}$~\cite{milbich2020diva}    % ECCV'20
        % CUB-200-2011
        & 69.2
        & 79.3 
        & -
        & 71.4
        % CARS-196
        & 87.6
        & 92.9
        & -
        & 72.2
        % SOP
        & 79.6 
        & 91.2
        & -
        & 90.6
        \\
    
    DCML$^{\text{512}}$~\cite{zheng2021compositional}  % CVPR'21
        % CUB-200-2011
        & 68.4 
        & 77.9
        & 86.1
        & 71.8
        % CARS-196
        & 85.2 
        & 91.8
        & 96.0
        & 73.9
        % SOP
        & \underline{79.8}
        & 90.8
        & 95.8
        & 90.8
        \\
    
    IBC$^{\text{512}}$~\cite{seidenschwarz2021learning}  % ICML'21
        % CUB-200-2011
        & \underline{70.3}
        & \underline{80.3}
        & \underline{87.6}
        & \underline{74.0}
        % CARS-196
        & \underline{88.1}
        & \underline{93.3}
        & \underline{96.2}
        & \underline{74.8}
        % SOP
        & \textbf{81.4}
        & \underline{91.3}
        & 95.9
        & \underline{92.6}
        \\
    
    % \midrule
    \rowcolor{Gray}
    HIST$^{\text{512}}$ (Ours)
        % CUB-200-2011
        & \textbf{71.4}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{81.1}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.3}
        & \textbf{88.1}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{74.1}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        % CARS-196
        & \textbf{89.6}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{93.9}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        & \textbf{96.4}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        & \textbf{75.2}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.3}
        % SOP
        & \textbf{81.4}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{92.0}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{96.7}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        & \textbf{92.8}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        \\
    
    % \midrule
    % % \midrule
    
    % \multicolumn{5}{l}{\textit{\textbf{Methods using SwAV~\cite{caron2020unsupervised}:}}}
    % & & & &
    % & & & &
    % \\
    
    % Grouplet$^{\text{512}}$~\cite{zhang2021learning}  % ICCV'21
    %     % CUB-200-2011
    %     & \underline{75.4}
    %     & \underline{83.4}
    %     & \underline{90.1}
    %     & \underline{76.4}
    %     % CARS-196
    %     & \underline{91.5}
    %     & \underline{94.8}
    %     & \underline{96.9}
    %     & \underline{77.6}
    %     % SOP
    %     & \underline{82.0}
    %     & \underline{92.7}
    %     & \underline{97.2}
    %     & \underline{91.1}
    %     \\
    
    % HGR-x1$^{\text{512}}$ (Ours)
    %     % CUB-200-2011
    %     & 
    %     & 
    %     & 
    %     & 
    %     % CARS-196
    %     & 
    %     & 
    %     & 
    %     & 
    %     % SOP
    %     & 
    %     & 
    %     & 
    %     & 
    %     \\
    
    % HGR-x2$^{\text{512}}$ (Ours)
    %     % CUB-200-2011
    %     & 
    %     & 
    %     & 
    %     & 
    %     % CARS-196
    %     & 
    %     & 
    %     & 
    %     & 
    %     % SOP
    %     & 
    %     & 
    %     & 
    %     & 
    %     \\
    
    
    % \rowcolor{Gray}
    % % \midrule
    % HGR-x4$^{\text{512}}$ (Ours)
    %     % CUB-200-2011
    %     & 
    %     & 
    %     & 
    %     & 
    %     % CARS-196
    %     & 
    %     & 
    %     & 
    %     & 
    %     % SOP
    %     & 
    %     & 
    %     & 
    %     & 
    %     \\

    \bottomrule
\end{tabular}
}
\caption{
Comparisons with state-of-the-arts under the standard evaluation settings.
%
% Retrieval and Clustering performance on CUB-200-2011, CARS-196, and SOP datasets.
%
Superscript denotes the embedding dimension.
%
For all compared methods, the results were quoted from the original paper.
%
For our method, we reported the average performance with 95\% confidence interval evaluated over 10 independent runs.
%
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{res_cub_cars_sop}
\vspace{+1mm}
\end{table*}

==> tables/res_inshop.tex <==
\begin{table}
\centering
\scriptsize
{
\begin{tabular}{
p{0.14\textwidth}
cccc} 
    \toprule
    \multirow{2}{*}{Method}
    & \multicolumn{4}{c}{In-Shop}
    \\
    \cmidrule(l){2-5}
    & R@1 & R@10 & R@20 & R@30 
    \\
    \midrule
    \midrule
    
    FashionNet$^{\text{4096}}$~\cite{liu2016deepfashion} % CVPR'16
        % In-Shop
        & 53.0 
        & 73.0 
        & 76.0 
        & 77.0
        \\
    
    A-BIER$^{\text{512}}$~\cite{opitz2018deep} % ICCV'17 -> TPAMI'18
        % In-Shop
        & 83.1 
        & 95.1 
        & 96.9 
        & 97.5
        \\

    ABE$^{\text{512}}$~\cite{kim2018attention} % ECCV'18
        % In-Shop
        & 87.3 
        & 96.7 
        & 97.9 
        & 98.2
        \\
        
    N.Softmax$^{\text{512}}$~\cite{zhai2018classification} % BMVC'19
        % In-Shop
        & 88.6 
        & 97.5 
        & 98.4 
        & \underline{98.8}
        \\

    MS$^{\text{512}}$~\cite{wang2019multi} % CVPR'19
        % In-Shop
        & 89.7 
        & 97.9
        & 98.5 
        & \underline{98.8}
        \\
        
    FastAP$^{\text{512}}$~\cite{cakir2019deep} % CVPR'19
        % In-Shop
        & 90.9 
        & 97.7 
        & 98.5
        & \underline{98.8}
        \\
    
    ProxyNCA++$^{\text{512}}$~\cite{teh2020proxynca++} % ECCV'20
        % In-Shop
        & 87.6
        & -
        & -
        & -
        \\
    
    ProxyAnchor$^{\text{512}}$~\cite{kim2020proxy} % CVPR'20
        % In-Shop
        & 91.5
        & 98.1
        & \underline{98.8}
        & -
        \\
    
    % MS+SEC$^{\text{512}}$~\cite{zhang2020deep}  % NeurIPS'20
    %     % In-Shop
    %     & 89.9 
    %     & 97.9 
    %     & \underline{98.8}
    %     & \underline{99.1}
    %     \\
    
    IBC$^{\text{512}}$~\cite{seidenschwarz2021learning}  % ICML'21
        % In-Shop
        & \underline{92.8}
        & \underline{98.5}
        & \textbf{99.1}
        & -
        \\
    
    
    \rowcolor{Gray}  
    HGR$^{\text{512}}$ (목표)
        % In-Shop
        & \textbf{93.1}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.2}
        & \textbf{98.8}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        & \textbf{99.1}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        & \textbf{99.2}\scalebox{0.7}{$\pm$}\scalebox{0.75}{0.1}
        \\
    
    \bottomrule
\end{tabular}
}
\caption{Retrieval performance on In-Shop dataset.
Superscript denotes the embedding dimension.
%
For all compared methods, the results are quoted from the original paper.
%
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.}
\label{res-inshop}
\end{table}



==> tables/res_larger_image.tex <==
\begin{table}
\caption{Image retrieval and clustering performances (\%) on CUB-200-2011, CARS-196, and SOP datasets. 
%  
우리는 10번 반복실험. 괄호 안의 숫자는 95\% confidence interval 의 margin of error. 
%
For all compared methods, the results are quoted from the original paper.
% , and "-" means that the result is not provided.
Superscript denotes the embedding size, and "$\dagger$" indicates that the model uses a larger input image (256$\times$256).
% The top-3 results are shown in bold, with the best in red, the second-best in blue, and the third-best in black.
The best results are marked in \textbf{bold}, and the second-best results are \underline{underlined}.
}
\label{result-larger-image}
\centering
% \scriptsize
\tiny
{
\begin{tabular}{
p{0.155\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering}p{0.0375\textwidth}
>{\centering\arraybackslash}p{0.0375\textwidth}
} 
    \toprule
    \multirow{2}{*}{Method}
    &  \multicolumn{4}{c}{CUB-200-2011}
    &  \multicolumn{4}{c}{CARS-196}
    &  \multicolumn{4}{c}{SOP}
    \\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    \cmidrule(l){10-13}
    & R@1 & R@2 & R@4 & R@8 
    & R@1 & R@2 & R@4 & R@8 
    & R@1 & R@10 & R@10$^{\text{2}}$ & R@10$^{\text{3}}$
    \\
    \midrule

    $^{\dagger}$HORDE$^{\text{512}}$~\cite{jacob2019metric} % ICCV'19
        % CUB-200-2011
        & 66.3
        & 76.7
        & 84.7
        & 
        % CARS-196
        & 83.9
        & 90.3
        & 94.1
        & 
        % SOP
        & 80.1
        & 91.3
        & 96.2
        & 
        \\
    
    $^{\dagger}$ProxyNCA\tiny{++}$^{\text{512}}$~\cite{teh2020proxynca++} % ECCV'20
        % CUB-200-2011
        & 69.0
        & 79.8
        & 87.3
        & 
        % CARS-196
        & 86.5
        & 92.5
        & 95.7
        & 
        % SOP
        & 80.7
        & 92.0
        & 96.7
        & 
        \\
        
    $^{\dagger}$ProxyAnchor$^{\text{512}}$~\cite{kim2020proxy} % CVPR'20
        % CUB-200-2011
        & 71.1
        & 80.4
        & 87.4
        & 
        % CARS-196
        & 88.3
        & 93.1
        & 95.7
        & 
        % SOP
        & 80.3
        & 91.4
        & 96.4
        & 
        \\
    
    \midrule

    HDML$^{\text{512}}$
        % CUB-200-2011
        & \underline{71.4} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \underline{81.1} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.3}
        & \underline{88.1} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \underline{92.7} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        % CARS-196
        & \underline{89.6} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \underline{93.9} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        & \underline{96.4} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        & \underline{97.8} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        % SOP
        & \underline{80.9} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & 
        & 
        & 
        \\
   
   \midrule
   
    $^{\dagger}$HDML$^{\text{512}}$
        % CUB-200-2011
        & \textbf{73.0} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.3}
        & \textbf{82.2} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \textbf{88.8} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \textbf{93.2} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        % CARS-196
        & \textbf{90.6} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \textbf{94.7} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & \textbf{96.9} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        & \textbf{98.2} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.1}
        % SOP
        & \textbf{80.9} \scalebox{0.8}{$\pm$}\scalebox{0.85}{0.2}
        & 
        & 
        & 
        \\
    
    \bottomrule
\end{tabular}
}
\end{table}



==> tables/robustness.tex <==
\begin{table}
\centering
\footnotesize
\begin{tabular}{
% p{0.16\textwidth}
% >{\centering}p{0.08\textwidth}
% >{\centering}p{0.08\textwidth}
% >{\centering\arraybackslash}p{0.05\textwidth}
lccc
}
    \toprule
    Input corruption
    & Baseline
    & TF-like
    & HIST
    % & Gain
    \\
    \midrule
    \midrule

    % \multicolumn{4}{l}{\textit{\textbf{Additive noise:}}}
    \textit{\textbf{Additive noise:}}
    & & &
    \\
    
    Uniform
        & 83.2 $\pm$ 0.1
        & 85.5 $\pm$ 0.1
        & \textbf{88.0 $\pm$ 0.1}
        % & \textbf{\textcolor{magenta}{(+4.8)}}
        \\
    
    Gaussian
        & 67.4 $\pm$ 0.3
        & 71.3 $\pm$ 0.2
        & \textbf{76.2 $\pm$ 0.3} 
        % & \textbf{\textcolor{magenta}{(+8.8)}}
        \\
    
    Salt \& Pepper
        & 56.2 $\pm$ 0.2
        & 58.6 $\pm$ 0.2
        & \textbf{68.6 $\pm$ 0.2}
        % & \textbf{\textcolor{magenta}{(+12.4)}}
        \\
    
    \midrule

    % \multicolumn{4}{l}{\textit{\textbf{Dropping pixels:}}}
    \textit{\textbf{Dropping pixels:}}
    & & &
    \\
    
    Cutout
        & 73.4 $\pm$ 0.3
        & 76.9 $\pm$ 0.1
        & \textbf{81.8 $\pm$ 0.3}
        % & \textbf{\textcolor{magenta}{(+8.4)}}
        \\
    
    Dropout
        & 61.3 $\pm$ 0.3
        & 65.2 $\pm$ 0.2
        & \textbf{72.5 $\pm$ 0.4}
        % & \textbf{\textcolor{magenta}{(+11.2)}}
        \\
    
    \midrule
    
    % \multicolumn{4}{l}{\textit{\textbf{Affine transformation:}}}
    \textit{\textbf{Affine transformation:}}
    & & &
    \\

    Perspective
        & 77.7 $\pm$ 0.2
        & 81.0 $\pm$ 0.2
        & \textbf{84.3 $\pm$ 0.2}
        % & \textbf{\textcolor{magenta}{(+6.6)}}
        \\

    Rotation
        & 69.4 $\pm$ 0.3
        & 73.7 $\pm$ 0.4
        & \textbf{78.3 $\pm$ 0.2}
        % & \textbf{\textcolor{magenta}{(+8.9)}}
        \\
    
    \midrule
    
    % \multicolumn{4}{l}{\textit{\textbf{Degrading image quality:}}}
    \textit{\textbf{Degrading image quality:}}
    & & &
    \\
    
    JPEG-compression
        & 72.6 $\pm$ 0.2
        & 74.0 $\pm$ 0.3
        & \textbf{79.7 $\pm$ 0.3}
        % & \textbf{\textcolor{magenta}{(+7.1)}}
        \\
    
    Gaussian blur
        & 64.7 $\pm$ 0.2
        & 69.3 $\pm$ 0.2
        & \textbf{75.9 $\pm$ 0.2}
        % & \textbf{\textcolor{magenta}{(+11.2)}}
        \\
    
    \bottomrule
\end{tabular}
\vspace{-1mm}
\caption{Robustness to \textit{unseen} input corruptions. We evaluated retrieval performance (R@1) with different input corruptions (not used for training) on CAR-196 dataset.
% The best results are marked in \textbf{bold}.
% , and the second-best results are \underline{underlined}.
}
\label{robustness}
\end{table}
